How to make qubits speak

This is a story about making quantum computers speak, and doing so in a quantum-native, compositional and meaning-aware manner. Recently we did question-answering with an actual quantum computer. We explain what we did, stress that this was all done in terms of pictures, and provide many pointers to the related literature. In fact, besides natural language, many other things can be implemented in a quantum-native, compositional and meaning-aware manner, and we provide the reader with some indications of that broader pictorial landscape, including our account on the notion of compositionality. We also provide some guidance for the actual execution, so that the reader can give it a go as well.

==> macros/preamble.tex <==
\oddsidemargin 10pt
\evensidemargin 10 pt
\topmargin -.5in
\headsep 20pt
\footskip 38pt
\textheight 8.9in
\textwidth 6.25in

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}
\usepackage{hyperref}
\usepackage{amsmath,amssymb}
\usepackage{xspace}
\usepackage{color}
\usepackage{epsfig}
\graphicspath{{.}{./figures/}}
\pagestyle{headings}
\usepackage{keycommand}
\usepackage{macros/tikzfig}
\input{macros/defs.tex}
\input{macros/tikzstyles.tex}
\input{macros/tikzfigures.tex}
\def\bR{\begin{color}{red}}
\def\bB{\begin{color}{blue}}
\def\bM{\begin{color}{magenta}}
\def\bC{\begin{color}{cyan}}
\def\bW{\begin{color}{white}}
\def\bBl{\begin{color}{black}}
\def\bG{\begin{color}{green}}
\def\bY{\begin{color}{yellow}}
\def\e{\end{color}\xspace}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}\par\noindent}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}\par\noindent}
\newcommand{\bec}{\begin{center}}
\newcommand{\eec}{\end{center}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}\par\noindent}
\newcommand{\beqa}{\begin{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray*}\par\noindent}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}\par\noindent}
\newcommand{\TODOb}[1]{\marginpar{\scriptsize\bB \textbf{TODO:} #1\e}}
\newcommand{\TODOm}[1]{\marginpar{\scriptsize\bM \textbf{TODO:} #1\e}}
\newcommand{\TODOd}[1]{\marginpar{\scriptsize\bG \textbf{TODO:} #1\e}}
\newcommand{\COMMb}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMm}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMd}[1]{\marginpar{\scriptsize\bG \textbf{COMM:} #1\e}}
\newcommand{\Kon}[1]{\marginpar{\scriptsize\bM \textbf{Konment:} #1\e}}

\def\QiNLP{Q${}^i$NLP}

==> macros/preamble2.tex <==
\oddsidemargin -15pt
\evensidemargin -15pt
\topmargin -.8in
\headsep 20pt
\footskip 38pt
\textheight 9.5in
\textwidth 6.95in

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}
\usepackage{hyperref}
\usepackage{amsmath,amssymb}
\usepackage{xspace}
\usepackage{color}
\usepackage{epsfig}
\graphicspath{{.}{./figures/}}
\pagestyle{headings}
\usepackage{keycommand}
\usepackage{macros/tikzfig}
\input{macros/defs.tex}
\input{macros/tikzstyles.tex}
\input{macros/tikzfigures.tex}
\def\bR{\begin{color}{red}}
\def\bB{\begin{color}{blue}}
\def\bM{\begin{color}{magenta}}
\def\bC{\begin{color}{cyan}}
\def\bW{\begin{color}{white}}
\def\bBl{\begin{color}{black}}
\def\bG{\begin{color}{green}}
\def\bY{\begin{color}{yellow}}
\def\e{\end{color}\xspace}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}\par\noindent}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}\par\noindent}
\newcommand{\bec}{\begin{center}}
\newcommand{\eec}{\end{center}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}\par\noindent}
\newcommand{\beqa}{\begin{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray*}\par\noindent}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}\par\noindent}
\newcommand{\TODOb}[1]{\marginpar{\scriptsize\bB \textbf{TODO:} #1\e}}
\newcommand{\TODOm}[1]{\marginpar{\scriptsize\bM \textbf{TODO:} #1\e}}
\newcommand{\TODOd}[1]{\marginpar{\scriptsize\bG \textbf{TODO:} #1\e}}
\newcommand{\COMMb}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMm}[1]{\marginpar{\scriptsize\bM \textbf{COMM:} #1\e}}
\newcommand{\COMMd}[1]{\marginpar{\scriptsize\bG \textbf{COMM:} #1\e}}
\newcommand{\Kon}[1]{\marginpar{\scriptsize\bM \textbf{Konment:} #1\e}}

\def\QiNLP{Q${}^i$NLP}
